Hyperparameter optimization of data-driven AI models on HPC systems

In the European Center of Excellence in Exascale computing "Research on AI- and Simulation-Based Engineering at Exascale" (CoE RAISE), researchers develop novel, scalable AI technologies towards Exascale. This work exercises High Performance Computing resources to perform large-scale hyperparameter optimization using distributed training on multiple compute nodes. This is part of RAISE's work on data-driven use cases which leverages AI- and HPC cross-methods developed within the project. In response to the demand for parallelizable and resource efficient hyperparameter optimization methods, advanced hyperparameter search algorithms are benchmarked and compared. The evaluated algorithms, including Random Search, Hyperband and ASHA, are tested and compared in terms of both accuracy and accuracy per compute resources spent. As an example use case, a graph neural network model known as MLPF, developed for the task of Machine-Learned Particle-Flow reconstruction in High Energy Physics, acts as the base model for optimization. Results show that hyperparameter optimization significantly increased the performance of MLPF and that this would not have been possible without access to large-scale High Performance Computing resources. It is also shown that, in the case of MLPF, the ASHA algorithm in combination with Bayesian optimization gives the largest performance increase per compute resources spent out of the investigated algorithms.

==> hypertuning_tables/asha_grid.tex <==
\begin{table}[htbp]
\centering
\footnotesize
\begin{tabular}{l|rrrrrrr}
\toprule
{} &       \#1 &       \#2 &       \#3 &       \#4 &       \#5 &       \#6 &       \#7 \\
\midrule
val\_loss                &   \textbf{1.0717} &   1.1000 &   1.1228 &   1.1349 &   1.1644 &   1.1674 &   1.1753 \\
val\_cls\_loss            &   \textbf{0.0106} &   0.0109 &   0.0111 &   0.0113 &   0.0116 &   0.0116 &   0.0117 \\
val\_reg\_loss            &   0.1675 &   0.1034 &   0.2333 &   0.1372 &   0.1178 &   \textbf{0.1000} &   0.1443 \\
val\_cls\_acc\_weighted    &   0.8478 &   0.8378 &   0.8266 &   0.8386 &   0.8301 &   0.8335 &   \textbf{0.8486} \\
\midrule
bin\_size                &  40 &  40 &  40 &  40 &  40 &  40 &  40 \\
distance\_dim            &  64 &  64 & 256 & 128 & 128 &  64 & 128 \\
ffn\_dist\_hidden\_dim     & 256 &  64 & 256 & 128 &  64 &  64 & 128 \\
ffn\_dist\_num\_layers     &   2 &   2 &   2 &   1 &   1 &   2 &   2 \\
num\_graph\_layers\_common &   3 &   3 &   4 &   3 &   2 &   3 &   3 \\
num\_graph\_layers\_energy &   4 &   3 &   3 &   2 &   2 &   2 &   2 \\
num\_node\_messages       &   1 &   1 &   1 &   1 &   1 &   1 &   1 \\
\bottomrule
\end{tabular}
\caption{Summary of top performing trials according to validation loss after hypertuning using the ASHA algorithm in a grid search setting. This search used the texttt{cms\_pf\_ttbar} dataset version 1.1.0.}
\label{asha_grid_table}
\end{table}

==> hypertuning_tables/asha_rs.tex <==
\begin{table}[htpb]
\centering
\footnotesize
\begin{tabular}{l|rrrrrrr}
\toprule
{} &       \#1 &       \#2 &       \#3 &       \#4 &       \#5 &       \#6 &       \#7 \\
\midrule

\bottomrule
\end{tabular}
\caption{Summary of top performing trials according to validation loss after hypertuning using the ASHA algorithm in a random search setting drawing 200 samples. This search used the full dataset containing all samples listed in table \ref{tab:samples}.}
\label{asha_rs_table}
\end{table}


==> hypertuning_tables/asha_scikit.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|rrrrrrr}
\br
{} &       \#1 &       \#2 &       \#3 &       \#4 &       \#5 &       \#6 &       \#7 \\
\midrule
val\_loss                &  \textbf{ 0.075032} &   0.075434 &   0.075870 &   0.076926 &   0.080376 &   0.082974 &   0.083737 \\
val\_cls\_loss            &   \textbf{0.000749} &   0.000753 &   0.000758 &   0.000768 &   0.000803 &   0.000829 &   0.000836 \\
val\_reg\_loss            &   0.023513 &   0.024625 &   0.027294 &   0.026401 &   0.024368 &   0.023276 &   \textbf{0.020109} \\
val\_cls\_acc\_weighted    &   0.940946 &   0.939746 &   0.942789 &   \textbf{0.944045} &   0.940729 &   0.939742 &   0.938667 \\
bin\_size                &  64 &  40 &  32 &  32 &  40 &  64 &  64 \\
distance\_dim            &  64 & 128 & 128 & 128 & 128 &  32 & 256 \\
ffn\_dist\_hidden\_dim     & 128 & 128 & 128 & 128 & 128 & 128 & 256 \\
ffn\_dist\_num\_layers     &   3 &   2 &   3 &   3 &   3 &   2 &   2 \\
num\_graph\_layers\_common &   3 &   3 &   3 &   3 &   2 &   2 &   1 \\
num\_graph\_layers\_energy &   2 &   2 &   1 &   1 &   1 &   4 &   3 \\
num\_node\_messages       &   3 &   2 &   1 &   1 &   3 &   2 &   4 \\
output\_dim              &  64 & 128 & 128 & 128 &  64 & 128 &  64 \\
\tr
\end{tabular}
\caption{Summary of top performing trials according to validation loss after hypertuning using the ASHA algorithm in combination with Bayesian optimization drawing 200 samples. This search used the full dataset containing all samples listed in table \ref{tab:samples} and consumed approximately 886.4 node-hours or, equivalently, about 56730 CPU core-hours.}
\label{tab:asha_scikit}
\end{table}


==> hypertuning_tables/bohb_cosinedecay.tex <==
\begin{table}[htbp]
\centering
\footnotesize
\begin{tabular}{l|rrrrrrr}
\toprule
{} &     \#1 &     \#2 &     \#3 &     \#4 &     \#5 &     \#6 &     \#7 \\
\midrule
val\_loss             & \textbf{1.0034} & 1.0569 & 1.0956 & 1.1581 & 1.1929 & 1.2479 & 1.3218 \\
val\_cls\_loss         & \textbf{0.0100} & 0.0105 & 0.0109 & 0.0115 & 0.0119 & 0.0124 & 0.0132 \\
val\_reg\_loss         & \textbf{0.1444} & 0.7239 & 0.5163 & 0.7085 & 0.7442 & 0.9475 & 0.2015 \\
val\_cls\_acc\_weighted & 0.8570 & 0.8544 & \textbf{0.8574} & 0.8321 & 0.8410 & 0.8032 & 0.8221 \\
\midrule
clip\_value\_low       & 0.0020 & 0.0095 & 0.0446 & 0.0073 & 0.0064 & 0.0231 & 0.0092 \\
dist\_mult            & 0.1209 & 0.1473 & 0.1542 & 0.1315 & 0.1495 & 0.1723 & 0.1619 \\
dropout              & 0.0163 & 0.0638 & 0.0513 & 0.1150 & 0.1156 & 0.4203 & 0.0163 \\
lr                   & 0.0011 & 0.0020 & 0.0011 & 0.0012 & 0.0013 & 0.0031 & 0.0014 \\
\bottomrule
\end{tabular}
\caption{Summary of top performing trials using a cosine decay learning rate schedule according to validation loss after hypertuning using the BOHB algorithm. This search used the \texttt{TTbar\_14TeV\_TuneCUETP8M1\_cfi} dataset and used approximately 98.4 node-hours, or 6298 CPU core-hours, of compute resources.}
\label{tab:bohb_cosinedecay}
\end{table}


==> hypertuning_tables/bohb_expdecay.tex <==
\begin{table}[htpb]
\centering
\footnotesize
\begin{tabular}{l|rrrrrrr}
\toprule
{} &     \#1 &     \#2 &     \#3 &     \#4 &     \#5 &     \#6 &     \#7 \\
\midrule
val\_loss             &   \textbf{1.0208} &   1.0761 &    1.1077 &   1.1189 &   1.1554 &   1.1666 &   1.1913 \\
val\_cls\_loss         &   \textbf{0.0102} &   0.0107 &    0.0110 &   0.0112 &   0.0115 &   0.0116 &   0.0119 \\
val\_reg\_loss         &   1.1464 &   0.9961 &    0.8574 &   0.5229 &   0.2573 &   \textbf{0.2181} &   0.2900 \\
val\_cls\_acc\_weighted &   0.8515 &   0.8578 &    0.8420 &   \textbf{0.8592} &   0.8561 &   0.8336 &   0.8365 \\
\midrule
clip\_value\_low       &   0.0254 &   0.0185 &    0.0297 &   0.0204 &   0.0336 &   0.0351 &   0.0328 \\
dist\_mult            &   0.1345 &   0.1335 &    0.0936 &   0.0497 &   0.0752 &   0.0823 &   0.0414 \\
dropout              &   0.1209 &   0.1184 &    0.1238 &   0.1268 &   0.0191 &   0.0154 &   0.0239 \\
expdecay\_decay\_steps & 700.0000 & 340.0000 & 1220.0000 & 130.0000 & 500.0000 & 490.0000 & 620.0000 \\
lr                   &   0.0025 &   0.0013 &    0.0023 &   0.0027 &   0.0016 &   0.0013 &   0.0011 \\
\bottomrule
\end{tabular}
\caption{Summary of top performing trials according to validation loss after hypertuning using the BOHB algorithm. These trials were run using an exponential decay learning rate schedule. This search used the \texttt{TTbar\_14TeV\_TuneCUETP8M1\_cfi} dataset and used approximately 105.5 node-hours, or 6750 CPU core-hours, of compute resources.}
\label{bohb_expdecay_table}
\end{table}
